Natural Language Can Help Bridge the Sim2Real Gap

The main challenge in learning image-conditioned robotic policies is acquiring a visual representation conducive to low-level control. Due to the high dimensionality of the image space, learning a good visual representation requires a considerable amount of visual data. However, when learning in the real world, data is expensive. Sim2Real is a promising paradigm for overcoming data scarcity in the real-world target domain by using a simulator to collect large amounts of cheap data closely related to the target task. However, it is difficult to transfer an image-conditioned policy from sim to real when the domains are very visually dissimilar. To bridge the sim2real visual gap, we propose using natural language descriptions of images as a unifying signal across domains that captures the underlying task-relevant semantics. Our key insight is that if two image observations from different domains are labeled with similar language, the policy should predict similar action distributions for both images. We demonstrate that training the image encoder to predict the language description or the distance between descriptions of a sim or real image serves as a useful, data-efficient pretraining step that helps learn a domain-invariant image representation. We can then use this image encoder as the backbone of an IL policy trained simultaneously on a large amount of simulated and a handful of real demonstrations. Our approach outperforms widely used prior sim2real methods and strong vision-language pretraining baselines like CLIP and R3M by 25 to 40%. See additional videos and materials at https://robin-lab.cs.utexas.edu/lang4sim2real/.

==> 03-problem_setup_0201.tex <==
In this work, we address the problem of few-shot visual imitation-learning: learning a visuomotor manipulation policy in the real world based on a few real-world demonstrations. We render this problem a sim2real learning problem assuming we gain access to a large amount of demonstration data from a simulator. More generally, we assume we have two learning domains: a prior $\priorD$ and target $\targetD$ domain. We assume we have a large amount of data from the prior domain including demonstrations for multiple tasks, $\goalT$, composed of sequences of pairs of images and action labels,  a language label description per demo ($l_{task}$), and language descriptions for some images ($l^{p}$). This data can be collected cheaply because it is generated by a simulator. We also assume access to some data in the, $\targetD$, including a few demonstrations for the task of interest, $\goalT$, also composed of sequences of pairs of images and action labels and a language label description per demo ($l_{task}$) and a few images of a second different task, $\languageT$, annotated with language descriptions ($l^{p}$).
The performance of a trained policy in $\goalT$ is our evaluation criteria, but we assume that data from $\targetD$ is significantly more expensive to collect because it corresponds to real-world data.
In the following, we explain further the different datasets we have access to in our problem.

\subsection{Action-labeled Data}
\label{sec:problem-setup:demos}
For each domain, we assume access to different amounts of expert demonstrations in the form of sequences of action-labeled images, and for different numbers of tasks. Each task is labeled with a language instruction, $l_{task}$.
We only have access to a few demonstrations ($<100$) on a \textit{single} target task, $\goalT$ in $D^{t}$, that we aim to learn a policy for. \textit{$\goalT$ is the only action-labeled visual data in $\targetD$} to which we have access. We also have access to a larger amount of action-labeled visual data in the prior domain, $\priorD$, from $k$ prior tasks $\priorT$, that we assume totaling several thousand demonstrations.
We assume that the target task, $\goalT$, is \textbf{not} one of the prior tasks $\priorT$. 
However, for \ouralgo{} to exploit the prior data to solve the target task, there must exist some similarities between $\goalT$ and $\priorT$. For instance, $\goalT \cup \priorT$ may all be of the same class of tasks, such as multi-step pick-and-place task compositions, but with different objects and containers across different subtasks.

Each demonstration is a sequence of tuples $(o_t, s_t, l_{task}, a_t)$, where $o_t \in \mathbb{R}^{128 \times 128 \times 3}$ is an RGB image observation, $s_t \in \mathbb{R}^{22}$ is the robot proprioceptive state (end-effector Cartesian position, the sine and cosine transforms of the joint position angles, and the continuous gripper closing state), and $a_t \in \mathbb{R}^{4}$ is the Cartesian-space xyz-delta action, plus the gripper closing continuous action.

\subsection{Paired Image and Language Data for Pretraining}
To leverage language in learning a domain-invariant representation, we assume access to two paired datasets of robot image observation and language scene description pairs: $\left( o^{p}, l^{p} \right)$ in $D^{p}$ and $\left( o^{t}, l^{t} \right)$ in $D^{t}$. The observations $o^{p}$ are from the action-labeled trajectories in tasks $T^{p}_{1:k}$ in $D^{p}$, and the observations $o^{t}$ are from action-labeled trajectories in a single task $T^{t}_{prior}$ in $D^{t}$, but crucially, $T^{t}_{prior} \ne T^{t}$, the target task we wish to transfer to---the two tasks involve manipulating different objects.

Given these two sets of image observations $O^{p}$ and $O^{t}$, we assume access to a language labeler that maps image observations to language scene descriptions. The language labeler, which can either be a programmatic function or a human, gives us paired image and language data that we use to learn our domain invariant representation. In our method, we use a programmatic function to label images with language. Note that these language \textit{scene descriptions} are different from the language \textit{instruction} associated with each task, $l_{task}$, in Section~\ref{sec:problem-setup:demos}.


==> 03-problem_setup_0420.tex <==
In this work, we address the problem of few-shot visual imitation-learning (IL): learning a visuomotor manipulation policy in the real world based on a few real-world demonstrations. We assume access to a large amount of simulation data and \rev{cast} few-shot IL as a sim2real problem. More concretely, we will render the few-shot IL problem as a $k+1$ multi-task IL problem: $k$ tasks from simulation and the few-shot task target in the real world. In general terms, we assume a \textit{source domain} in which data can be acquired cheaply and a \textit{target domain} where data is expensive to collect.

In our setting, we consider access to three datasets across these two domains: $\priorD$, which spans multiple tasks in the source domain, $\targetDtargetT$ which contains a small number of demonstrations of the target task in the target domain we want to transfer to, and $\targetDpriorT$ which consists of a few demonstrations of \textit{another} task in the target domain that we perform pretraining on. Thus, we assume that $|\priorD| >> |\targetDtargetT| \approx |\targetDpriorT|$, due to how expensive target domain data collection is (such as in the real world). We make two assumptions about the two domains. First, we assume the source and target tasks are all of the same general structure, such as multi-step pick-and-place task compositions, but with different objects and containers across different subtasks. Otherwise, transfer would be infeasible in the low-data regime if the source and target domain tasks lack similarity. Second, to train a common policy for both domains, we assume the domains share state and action space dimensionality. We make no further assumptions about the similiarity between the two domains.

All of our datasets are in the form of expert trajectories. Each trajectory, $\tau = \{(I_t, s_t, [a_t, l_t], l_{task} )\}$, is a sequence of tuples containing an image observation, $I_t$ ($128\times128$ RGB), robot proprioceptive state, $s_t$ (end effector position and joint angles), and a language instruction of the task, $l_{task}$. Note that $l_{task}$ is the same over all timesteps of all trajectories in a given task. $[a_t, l_t]$ denotes that a trajectory may optionally also include robot actions (in which case we consider the trajectory a full demonstration) and/or a language description of the image $I_t$. In the following sections, we identify with $\tau[L]$ a trajectory with language descriptions, $l_t$, but no actions, $a_t$. Similarly, $\tau[A]$ is a full demonstration with actions, $a_t$, but no language descriptions, $l_t$, and $\tau[AL]$ is a demonstration that contains both actions, $a_t$, and language, $l_t$. In the following sections, we refer to any trajectories with action labels $\left( \tau[A], \tau[AL] \right)$ as \textit{demonstrations}.

The language labels for images \rev{can be automatically generated from} a programmatic function that maps image observations to language scene descriptions depending on the relative position between the robot and the objects in the scene. \rev{We describe these language labels and how to automatically collect them in Section~\ref{sec:method:langlabeling}.} Note that these language \textit{scene descriptions}, $l_t$, are different from the language \textit{instruction} associated with each task, $l_{task}$.

We assume that $\priorD$ contains demonstration trajectories with both action labels and language descriptions in each transition $\tau[AL]$, $\targetDpriorT$ contains trajectories with image language labels $\tau[L]$, and $\targetDtargetT$ contains demonstrations with action labels and no language descriptions $\tau[A]$. Different data elements, datasets, and types of trajectories will be used during pretraining and policy few-shot training: during pretraining, we use $\tau[L]$ image-language $(I_t, l_t)$ pairs from $\priorD \cup \targetDpriorT$. During policy learning, we use $\tau[A]$ data: $(\rev{I_t}, s_t, a_t, l_{task})$ tuples from $\priorD \cup \targetDtargetT$. In the next section, we explain how these two steps are defined for \ouralgo{}.


==> 05-experimental-setup_0420.tex <==
We evaluate \ouralgo{} in two settings: a \texttt{sim2sim} setting where we test the transfer abilities between two simulated domains with visual and physical differences, and the \texttt{sim2real} setting, where the few shot IL is defined in the real world and we use simulation to address the data scarcity. \texttt{Sim2sim} serves as a platform to evaluate in depth the behavior of \ouralgo{} with a fully controlled gap, while \texttt{sim2real} is our domain of interest for this work. We will use three task suites that we explain below. See Appendix for detailed frame rollouts of each task. In a slight overload of notation from Sec.~\ref{sec:problem-setup}, here we use $\priorD$ to denote the source domain and $\targetD$ to denote the target domain. 

\subsection{\texttt{Sim2Sim} and \texttt{Sim2Real} Environment Differences}
% \label{sec:exp:sim2simdiff}
\label{sec:exp:sim2sim-sim2real-diff}
In \texttt{sim2sim}, $\priorD$ and $\targetD$ are both sim environments with large differences in camera point-of-view (third person vs. first person), joint friction, and damping.
% \begin{enumerate}
%     \item \textbf{Camera point-of-view}: $\priorD$ image observations are third person (looking toward the robot), and $\targetD$ image observations are first person (over the shoulder), a large viewing angle change.
%     \item \textbf{Friction and Damping}: Joint friction and damping coefficients are $5 \times$ and $50\times$ higher in $\targetD$ than $\priorD$, which changes significantly the dynamics.
% \end{enumerate}
% \subsection{\texttt{sim2real} Environment Differences}
% \label{ss:s2rdiffs}
In the \texttt{sim2real} setting,
% in contrast with prior work that requires significant engineering to reduce differences between the sim $\priorD$ and real $\targetD$ environment,
we employ a setup with a wide \texttt{sim2real} gap that we aim to bridge using language that includes differences in control frequency, task goals, visual observation appearance, objects, and initial positions.
% \begin{enumerate}
%     \item \textbf{Control frequency}: The simulated $\priorD$ policy runs at 50Hz while the real world $\targetD$ policy runs at 2Hz.
%     \item \textbf{Objects}: The objects on the scene in each task differ between simulation and real data, except the robot itself.
%     \item \textbf{Visual Observation}: Backgrounds and camera angles are markedly different between the two domains.
%     \item \textbf{Initial positions}: The initial object and robot positions are different across sim and real.
%     % \item \textbf{Action magnitude}: Real robot x, y, and z action are restricted so each are $\le 1$, and higher values are scaled before being executed. 
% \end{enumerate}
More details between the two environments in \texttt{sim2sim} and \texttt{sim2real} can be found in the Appendix.

\subsection{Evaluation Metrics}
\label{sec:exp:metric}
Across all sim2sim and sim2real experiments, we measure task success rate. In sim2real, this is calculated through ten evaluation trials for each of two seeds per task, for a total of 20 trials per table entry. In each set of ten trials, we place the object in the same ten initial positions and orientations, evenly distributed through the range of valid initial object positions. In sim2sim, we also run two seeds per setting and take a success rate averaged over 720 trials between the two seeds in the final few hundred epochs of training.
% and average the success rate on twelve evaluation trial every ten epochs between 300 and 600 epochs (for a total of 720 trials).

\subsection{Data}
\subsubsection{Environments} For each of our tasks, we design simulation environments on top of Robosuite~\citep{zhu2020robosuite} in Mujoco~\citep{todorov2012mujoco}. For the real environment, we use Operational Space Control~\cite{khatib1987unified} to control the position of the end-effector of the robot in Cartesian space. In both simulation and real, we work with a 7-D0F Franka Emika Panda arm and use a common action space consisting of the continuous xyz delta displacement and a continuous gripper closure dimension (normalized from $[-1, 0]$).  The robot proprioception space is 22-dimensional, consisting of the robot's xyz end-effector position, gripper state, and sine and cosine transformations of the 7 joint angles. The image observation space is $128 \times 128$ RGB images.

\subsubsection{Overview of Tasks} For each task suite, we collect data from simulated domain $\priorD$ and real target domain $\targetD$ (for \texttt{sim2real}) or sim target domain $\targetD$ (for \texttt{sim2sim}). All demonstrations in sim and real are collected with a scripted policy (see Appendix for further details). Sim trajectories range from 200-320 timesteps long, operated at \SI{50}{\hertz}, while real trajectories run at \SI{2}{\hertz} and range from 18-45 timesteps. Our three task suites allow us to test the effectiveness of \ouralgo{} for sim2real in a wide variety of control problems ranging from simple stacking in task suite 1, to multi-step long-horizon pick and place in task suite 2, to deformable, hard-to-simulate objects in task suite 3.

\begin{figure}[t!]
\centering
\includegraphics[width=0.32\linewidth]{figs/task_images/simppm2.jpg}%
\hfill%
\includegraphics[width=0.32\linewidth]{figs/task_images/simppx212.jpg}%
\hfill%
\includegraphics[width=0.32\linewidth]{figs/task_images/simww12.jpg}\\
\vspace{5pt}
\includegraphics[width=0.32\linewidth]{figs/task_images/simppt2.jpg}%
\hfill%
\includegraphics[width=0.32\linewidth]{figs/task_images/simppx2t2.jpg}%
\hfill%
\includegraphics[width=0.32\linewidth]{figs/task_images/simwwt2.jpg}\\
\vspace{5pt}%
\includegraphics[width=0.32\linewidth]{figs/task_images/realpp.jpg}%
\hfill%
\includegraphics[width=0.32\linewidth]{figs/task_images/realppx2.jpg}%
\hfill%
\includegraphics[width=0.32\linewidth]{figs/task_images/realw.jpg}\\
\caption{The columns depict the three task suites while each row represents an image domain. \textit{\rev{Rows from Top to Bottom}:} Simulation $\priorD$, \texttt{sim2sim} $\targetDtargetT$, \texttt{sim2real} $\targetDtargetT$\rev{.} \textit{\rev{Columns from} Left to Right:} Stack Object, Multi-step Pick and Place, and Wrap Wire tasks. While similar enough to transfer prior knowledge between them, our $\priorD$ and $\targetD$ task versions \rev{have} a considerable gap (Sec.~\ref{sec:exp:sim2sim-sim2real-diff}) that we are able to bridge using language as regularization for the image representations.}  
\label{fig:tasks}
\end{figure}

%%%%%%%%%%%%%%
%%% TASK 1 %%%
%%%%%%%%%%%%%%
\subsection{Task Suite 1: Stack Object}
\label{sec:exp:stack}
In our first suite of tasks, the robot must move an object to a target. In the simulated domain $\priorD$, the target is on top of a wooden coaster, and there are four objects: milk carton, soda can, bread, and cereal box, which correspond to the four tasks. Both the object and coaster positions are randomized over the entire workspace. We collect and train on $400$ demonstrations per task ($1600$ total) as our $\priorD$ simulation data.
\begin{table*}[htbp]
  \centering
  \caption{\texttt{sim2real}: \rev{Performance by Number of Target Task Demonstrations}}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{cccccccccccccccc}
    \toprule
    Pretraining & \multicolumn{3}{c}{Action-labeled Data} &  \multicolumn{3}{c}{Stack Object} & \multicolumn{6}{c}{Multi-step Pick and Place} & \multicolumn{3}{c}{Wrap Wire}\\
    \cmidrule(r{4pt}){2-4} \cmidrule(l){5-7} \cmidrule(l){8-13} \cmidrule(l){14-16}
    & Sim & \multicolumn{2}{c}{Real} & \multicolumn{3}{c}{Success Rate \rev{(\%)}} & \multicolumn{3}{c}{Success Rate \rev{(\%)}} & \multicolumn{3}{c}{Subtasks Completed} & \multicolumn{3}{c}{Success Rate \rev{(\%)}} \\
    \cmidrule(l){5-7}\cmidrule(l){8-10}\cmidrule(l){11-13} \cmidrule(l){14-16}
    &  $\priorD$ &  $\targetDtargetT$ &  $\targetDpriorT$& 25 & 50 & 100 & 25 & 50 & 100 & 25 & 50 & 100 & 25 & 50 & 100 \\
    \midrule 
    
    None ($\targetD$ data only) & -- & \ding{51} & \ding{51} & 45 & 30 & 65 & 40 & 20 & 30 & 1.15 & 0.9 & 1.15 &  25 & 45 & 35\\
     None ($\priorD + \targetD$ data) & \ding{51} & \ding{51} & \ding{51} & 20 & 55 & 25 & 45 & 30 & 50 & 1.25 & 1.2 & 1.4 & 15 & 30 & 30 \\
    \midrule
    \rev{MMD} & \rev{\ding{51}} & \rev{\ding{51}} & \rev{\ding{51}} & \rev{35} & \rev{30} & \rev{40} & \rev{70} & \rev{45} & \rev{35} & \rev{\textbf{1.65}} & \rev{1.25} & \rev{1.2} & \rev{15} & \rev{0} & \rev{20} \\
    \rev{Domain Random.} & \rev{\ding{51}} & \rev{\ding{51}} & \rev{\ding{51}}  & \rev{25} & \rev{45} & \rev{60} & \rev{15} & \rev{15} & \rev{20} & \rev{0.9} & \rev{0.55} & \rev{0.85} & \rev{0} & \rev{5} & \rev{5} \\
    \rev{ADR+RNA} & \rev{\ding{51}} & \rev{\ding{51}} & \rev{\ding{51}} & \rev{15} & \rev{10} & \rev{20} & \rev{50} & \rev{5} & \rev{50} & \rev{1.35} & \rev{0.7} & \rev{1.25} & \rev{15} & \rev{10} & \rev{20} \\
    
    \midrule
    Lang Reg. (ours) & \ding{51} & \ding{51} & -- & 50 & 55 & \textbf{85} & 55 & \textbf{80} & \textbf{95} & 1.2 & \textbf{1.8} & \textbf{1.95} & 25 & \textbf{50} & 55\\
    Lang Dist. (ours) & \ding{51} & \ding{51} & -- & 30 & 65 & 70 & 25 & 50 & 65 & 0.95 & 1.4 & 1.5 & 15 & 25 & 60  \\
    Stage Classif. & \ding{51} & \ding{51} & -- & 70 & 60 & 70 & 20 & 60 & 85 & 0.9 & 1.5 & 1.8 & 15 & 20 & \textbf{70} \\
    \midrule
    CLIP (frozen) & \ding{51} & \ding{51} & \ding{51} & 30 & 25 & 35 & 25 & 45 & 35 & 0.55 & 0.95 & 0.95 & \textbf{35} & 40 & 45\\ 
    R3M (frozen) & \ding{51} & \ding{51} & \ding{51} & \textbf{80} & \textbf{70} & 80 & \textbf{75} & 75 & 85 & 1.6 & 1.55 & 1.75 & 30 & 25 & 20\\
    \bottomrule
  \end{tabular}
  }
  \label{tab:real}
\end{table*}

\begin{table*}[htbp]
  \centering
  \setlength{\tabcolsep}{0.2em}
  \caption{\texttt{sim2sim}: Success Rate by Task (\%)}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{ccccccccccccccc}
    \toprule
     
     Pretraining & \multicolumn{5}{c}{Stack Object} & \multicolumn{5}{c}{Multi-step Pick and Place} & Wrap Wire \\
    \cmidrule(l){2-6}
    \cmidrule(l){7-11}
    \cmidrule(l){12-12}
    & 1 & 2 & 3 & 4 & avg & 1 & 2 & 3 & 4 & avg & 1\\
    \midrule
    None ($\targetD$ data only) & $15.2 \pm 6.5$ & $18.9 \pm 6.7$ & $31.9 \pm 8.5$ & $25.4 \pm 9.2$ & $22.9$ & $20.8 \pm 7.5$ & $17.7 \pm 4.4$ & $16.3 \pm 5.0$ & $17.3 \pm 8.1$ & $18.0$ & $69.2 \pm 8.3$ \\
    None ($\priorD + \targetD$ data)  & $22.5 \pm 9.2$ & $32.3 \pm 9.8$ & $37.9 \pm 8.8$ & $29.2 \pm 8.3$ & $30.5$ & $28.4 \pm 10.9$ & $31.3 \pm 10.7$ & $13.9 \pm 5.5$ & $27.8 \pm 10.2$ & $25.4$ & $82.1 \pm 6.8$  \\
    \midrule
    Lang Reg. (ours) & $20.6 \pm 8.1$ & \boldmath{$57.3 \pm 8.1$} & $63.1 \pm 7.7$ & \boldmath{$32.5 \pm 6.3$} & $43.4$ & $54.0 \pm 7.2$ & \boldmath{$62.5 \pm 12.1$} & $76.0 \pm 8.7$ & $58.5 \pm 9.3$ & $62.8$ & $90.7 \pm 5.4$   \\
    Lang Dist. (ours) & $23.8 \pm 5.4$ & \boldmath{$57.3 \pm 10.6$} & $66.9 \pm 5.6$ & $27.9 \pm 10.8$ & $44.0$ & \boldmath{$65.5 \pm 13.1$} & $56.7 \pm 9.9$ & \boldmath{$78.6 \pm 5.1$} & $54.4 \pm 11.5$ & \boldmath{$63.8$} & $90.0 \pm 5.0$   \\
    Stage Classif. & \boldmath{$30.4 \pm 10.4$} & $52.7 \pm 6.0$ & \boldmath{$67.5 \pm 8.3$} & $27.9 \pm 7.1$ & \boldmath{$44.6$} & $63.1 \pm 9.9$ & $62.1 \pm 9.3$ & $55.4 \pm 8.5$ & \boldmath{$67.7 \pm 9.7$} & $62.1$ & \boldmath{$91.4 \pm 3.6$}   \\
    \midrule
    CLIP (frozen) & $1.7 \pm 0.4$ & $1.9 \pm 1.9$ & $3.8 \pm 2.5$ & $4.0 \pm 2.7$ & $2.9$ & $36.1 \pm 14.3$ & $39.9 \pm 8.9$ & $28.8 \pm 8.9$ & $48.4 \pm 11.9$ & $38.3$ & $75.6 \pm 7.7$  \\
    R3M (frozen) & $4.5 \pm 3.3$ & $9.0 \pm 4.8$ & $19.8 \pm 6.9$ & $15.4 \pm 5.4$ & $12.2$ & $49.4 \pm 11.6$ & $36.5 \pm 11.9$ & $47.0 \pm 14.1$ & $56.0 \pm 10.0$ & $47.2$ & $90.2 \pm 4.4$ \\
    \bottomrule
  \end{tabular}
  }
  \label{tab:sim}
\end{table*}
\subsubsection{\textbf{\texttt{sim2sim}}} For \texttt{sim2sim} experiments on this task suite, we define a new $\targetD$ simulated environment with differences from $\priorD$ as enumerated in Sec.~\ref{sec:exp:sim2sim-sim2real-diff}. Policies are trained with the 1600 $\priorD$ demonstrations and 100 target task $\targetDtargetT$ demonstrations. $\targetDpriorT$ consists of stacking trajectories but with a different one of the four objects than in $\targetDtargetT$.
%Note that $\targetD$, like $\priorD$, has the same four tasks that involve manipulating the four objects.  i thought this was kind of confusing

\subsubsection{\textbf{\texttt{sim2real}}} For \texttt{sim2real}, $\priorD$ remains the same as \texttt{sim2sim}. $\targetD$ is a real world environment in which the object is randomly placed on the left mat and the goal is to move the object onto the right mat and open the gripper by the end of 20 timesteps. As a real world prior task $\targetDpriorT$, we collect 50 trajectories of moving a small paper box from the left to the right mat, while $\targetDtargetT$ involves moving a carrot. %Our method pretrains on the images from these 50 prior task trajectories without any other $\targetD$.

%%%%%%%%%%%%%%
%%% TASK 2 %%%
%%%%%%%%%%%%%%

\subsection{Task Suite 2: Multi-step Pick and Place}
Our second suite of tasks is longer-horizon. In simulation, the robot must first put an object in the pot, then grasp the pot by its handle and move it onto the stove. We categorize this as a 2-step pick-and-place task. We use the same four object-task mappings from Sec.~\ref{sec:exp:stack}. The object, pot, and stove locations are all randomized within a quadrant of the workspace. Since this task is longer horizon, we train on more data---$1,400$ trajectories per task in $\priorD$.

\subsubsection{\textbf{\texttt{sim2sim}}} Similar to the stacking task, in the \texttt{sim2sim} setting, we define a new $\targetD$ environment with differences from $\priorD$ enumerated in Sec.~\ref{sec:exp:sim2sim-sim2real-diff} and evaluate over the four tasks when given $100$ target-task $\targetDtargetT$ demonstrations. $\targetDpriorT$ contains a different task from the one in $\targetDtargetT$.


\subsubsection{\textbf{\texttt{sim2real}}} In the \texttt{sim2real} setup, $\priorD$ remains the same, while $\targetD$ is the real task of putting a carrot into a bowl, then putting the bowl onto a plate (see Fig.~\ref{fig:tasks}), and ending with the gripper open after 50 timesteps. $\targetDpriorT$ data consists of 50 trajectories, but involving a wooden block instead of a carrot. In addition to success rate (Section~\ref{sec:exp:metric}), we measure average number of subtasks completed, allowing partial credit if the robot only succeeds in placing the carrot in the bowl, but not the bowl on the plate.

\subsection{Task Suite 3: Wrap Wire}
Our final suite of tasks involves wrapping a long deformable wire around a fixed object. In simulation $\priorD$, we approximate a wire with a chain of spheres connected with free joints and the task is to wrap the chain around a fixed cylinder (see Fig.~\ref{fig:tasks}). A trajectory is successful if the first link of the chain has traveled $\geq \frac{5\pi}{3}$ radians ($5/6$ths of a full revolution) around the cylinder. Our simulation data consists of two tasks: wrapping counterclockwise and clockwise. The initial position of the end of the chain is randomized over a region to the left of the cylinder. $\priorD$ contains 400 trajectories per task. 

\subsubsection{\textbf{\texttt{sim2sim}}} For our $\targetD$ sim environment, we again apply the changes specified in Sec.~\ref{sec:exp:sim2sim-sim2real-diff}. We additionally swapped the spheres for capsules and changed the color and texture of the table, robot arm, and objects. This task involves a wider sim2sim gap, given additional visual changes and dynamics changes. We collect 100 trajectories for $\targetDpriorT$ that involves wrapping clockwise instead of counterclockwise in $\targetDtargetT$.

\subsubsection{\textbf{\texttt{sim2real}}} In our \texttt{sim2real} experiments, the target task $\targetDtargetT$ is to first grasp the plug, then wrap the cord around the base of a blender in the middle of the workspace, and finally put the plug down, similar to what one might do before putting the appliance away. For real world prior task $\targetDpriorT$ data, we collect 50 trajectories of a similar wrapping task, except the plug, cord, and blender are replaced by a wooden block, ethernet cable, and spool, respectively.
 Like the sim environment, we define success if the following two conditions are met: (1) the plug travels $\geq \frac{5 \pi }{3}$ radians around the blender, and (2) the plug is placed and the gripper is open at the end of 50 timesteps. 

\subsection{Baselines}
To evaluate the effectiveness of \ouralgo{}, we consider two sets of baselines: non-pretrained baselines where the CNN is initialized from scratch, and baselines with pre-trained visual encoders.
For the non-pretrained baselines, we examine training with only $\targetD$ data, and training with both $\priorD$ and $\targetD$ data. This enables us to understand the benefits of our proposed training procedure.
\rev{We also compare to three popular prior sim2real approaches:}
\begin{itemize}
    \item \rev{MMD~\cite{tzeng2014deep}, which aims to minimize the distance between the means of all sim images and all real images of a batch to prevent the real images from being out-of-distribution relative to the sim images.}
    \item \rev{Domain randomization~\cite{tobin2017domain} of the colors, textures, and physics of the $\priorD$ environment.}
    \item \rev{Automatic Domain Randomization with Random Network Adversary (ADR+RNA)~\cite{openai2019solving}, which keeps increasing/decreasing domain randomization bounds depending on the agent's performance, and also introduces a randomly initialized network for each trajectory to inject correlated noise into the agent's action conditioned on the state input.}
\end{itemize}
For the pretrained baselines, we consider two strong foundation models as the visual backbone, CLIP~\cite{radford2021learning} and R3M~\cite{nair2022r3m}, commonly used visual representations for robotics that are, like our approach, also shaped by language descriptions of images/videos. %, as both are commonly used visual representations for robotics and were shaped by language descriptions of images/videos.

Since our method uses extra language labels during pretraining that the baselines do not have access to, in all our experiments, we give all baselines an augmented $\targetDpriorT$ dataset that includes action-labeled demonstrations, in addition to the target task, $\targetDtargetT$. \textit{Note that our method is not given $\targetDpriorT$ action-labeled data}: it is trained only on $\targetDpriorT$ images with language labels during image-language pretraining (Sec.~\ref{sec:method:imglangpt}) but not during BC policy learning. Therefore, the baselines in a sense serve as upper bounds as they are given $\left| \targetDpriorT \right| = 50$ additional action-labeled demonstrations. In other words, during policy learning, the baselines train on action-labeled demonstrations from $\priorD \cup \targetDpriorT \cup \targetDtargetT$ while ours are only trained on $\priorD \cup \targetDtargetT$. For each task, we train and evaluate at 3 different amounts of $\targetDtargetT$ demonstrations: 25, 50, 100.

\subsection{Our Method Variants and Ablations}
\label{exp-results:method-ablation}
In our evaluations, we compare language regression (Section~\ref{sec:method:lang-reg}) and language distance (Section~\ref{sec:method:lang-dist}), the two pretraining variants of our approach. We also ablate away the effects of language on our pretraining approach in a method called ``stage classification,'' where each unique language description is assigned a one-hot vector, and the task is to predict the one-hot vector given the image.

==> 05-experiments_0201.tex <==
To investigate the effectiveness of our method, we pose the following questions:
\begin{enumerate}[start=1,label={Q\arabic*:}]
    \item Can \ouralgo{} help bridge a wide sim2real gap involving large differences in visual appearance, scene objects, task goals, and robot control frequency?
    \item How does \ouralgo{} compare to prior vision-language pretrained representations that have demonstrated success in downstream robotics applications?
    \item What is the impact of language in learning shared representations as opposed to to similar non-language based domain-specific pretraining?
    \item How does pretraining via directly predicting language embeddings compare to distance learning, in which the CNN is encouraged to maintaining the BLEURT similarity between language and images?
    % \item Can \ouralgo{} help with sim2real transfer even on tasks that are difficult to faithfully simulate with high fidelity, such as manipulating deformable objects?
\end{enumerate}

We evaluate these questions across three task suites: (1) stacking an object on another, (2) cooking/serving food (multi-step pick and place), and (3) wrapping a cord around an appliance. For each task suite, we evaluate in both the sim2sim and sim2real settings. 

\subsection{Sim2Sim Environment Differences}
\label{sec:exp:sim2simdiff}
In sim2sim, the two sim environments $D^{(1)}$ and $D^{(2)}$ have the following differences:
\begin{enumerate}
    \item \textbf{Camera point-of-view}: $D^{(1)}$ image observations are third person (looking toward the robot), and $D^{(2)}$ image observations are first person (looking outward from above the robot arm's shoulder).
    \item \textbf{Friction and Damping}: Joint friction and damping coefficients are $5 \times$ and $50\times$ higher in $D^{(2)}$ than $D^{(1)}$.
    \item \textbf{Visual appearance}: For task 3, wrap wire, attributes including object and cylinder shape/color as well as table and gripper texture/color differ. 
\end{enumerate}

\subsection{Sim2Real Environment Differences}
\label{ss:s2rdiffs}
The sim and real environments share state and action space dimensionality to enable a single policy to fit to data from both domains, but compared to prior work that requires significant engineering to reduce differences between the sim $(D^{(1)})$ and real $(D^{(2)})$ environment, we employ a setup with a wide sim2real gap including the following factors:
\begin{enumerate}
    \item \textbf{Control frequency}: The simulated $D^{(1)}$ policy runs at 50Hz while the real world $D^{(2)}$ policy runs at 2Hz.
    \item \textbf{Objects}: The objects on the scene in each task differ between simulation and real data, except the robot itself.
    \item \textbf{Visual Observation}: Backgrounds and camera angles are markedly different between the two domains.
    \item \textbf{Initial positions}: The initial object and robot positions are different across sim and real.
    \item \textbf{Action magnitude}: Real robot  x, y, and z action are restricted so each are $\le 1$, and higher values are scaled before being executed. 
\end{enumerate}

\subsection{Baselines}
To evaluate the effectiveness of \ouralgo{}, we consider two sets of baselines: non-pretrained baselines where the CNN is initialized from scratch, and pre-trained baselines where the CNN is taken from recent vision+language works.
For the non-pretrained baselines, we examine training with only $D^{(2)}$ data, and training with both $D^{(1)}$ and $D^{(2)}$ data.
For the pretrained baselines, we compare with using frozen CLIP~\cite{radford2021learning} and R3M~\cite{nair2022r3m} as the visual backbone, as both are commonly used visual representations for robotics that were shaped by language descriptions of images/videos.

In all our experiments, all baselines (non-pretrained and pretrained) are given access to $D^{(2)}$ action-labeled data from two tasks: the target task $T^{(2)}$ and prior task $T^{(2)}_{prior}$. Crucially, our method, on the other hand, is only given action-labeled data for $T^{(2)}$. \textit{Our method is not given $T^{(2)}_{prior}$ action-labeled data} because it was trained on $T^{(2)}_{prior}$ images (with language labels) during image-language pretraining (Section~\ref{sec:method:imglangpt}). Therefore, the baselines in a sense serve as upper-bounds because they are given 50 additional trajectories of action-labels that our method never uses.

For each task, our experimental tables show results split by $x$ number of $T^{(2)}$ trajectories, where $x \in \{25, 50, 100\}$ (shown as columns under each performance metric). This means that in terms of $D^{(2)}$ action-labeled data, all baselines are trained on $x+50$ trajectories from $D^{(2)}$ ($x$ from $T^{(2)}$ and $50$ from $T^{(2)}_{prior}$), while our method is only trained on the $x$ action-labeled trajectories from $T^{(2)}$.

% (Explanation of the baselines): Note that the $D^{(2)}$-only baseline is only trained on the 100 trajectories of the target task in $D^{(2)}$, plus 50 trajectories of a prior task in $D^{(2)}$, $T^{(2)}_{prior}$ that our method pretrained on. The key difference is that while our method used $T^{(2)}_{prior}$ data without action labels but instead with language labels, all the baselines have access to $T^{(2)}_{prior}$ \textit{action}-labeled data. 

\subsection{Data}
Environments: For each of our tasks, we design simulation environments on top of robosuite~\citep{zhu2020robosuite} in mujoco~\citep{todorov2012mujoco}. For the real environment, we use Operational Space Control from deoxys. In both simulation and real, we work with a 7DOF Franka Emika Panda arm.

Both the sim and real environments have continuous xyz delta action space, and the gripper dimension is also continuous, ranging from $[-1, 0]$ to control the amount the gripper should be closed. The image observation space is $128 \times 128$ RGB images, and the state space is 22-dimensional, consisting of the robot's xyz end-effector position, gripper state, and sine and cosine transformations of the 7 joint angles.

For each task suite, we collect data from two domains: simulated domain $D^{(1)}$ and target domain $D^{(2)}$ (which is either another simulated domain or the real domain depending on whether we are doing sim2sim or sim2real transfer). All of our demonstrations in sim and real are collected with a scripted policy. Sim trajectories range from 200-320 timesteps long, as they operate at 50Hz, while real trajectories run at 2Hz and range from 18-45 timesteps in horizon length.

% All demonstrations are collected by a scripted policy. In both sim and real, we use xyz delta control. This is OSC position controller in deoxys~\cite{} in real. (See Appendix~\ref{blah} for details of the scripted policy.) Our sim environment is implemented in mujoco~\cite{} on top of the robosuite~\cite{} framework.

%%%%%%%%%%%%%%
%%% TASK 1 %%%
%%%%%%%%%%%%%%

\begin{figure}[t!]
\centering
\includegraphics[width=0.32\linewidth]{example-image-a}%
\hfill%
\includegraphics[width=0.32\linewidth]{example-image-a}%
\hfill%
\includegraphics[width=0.32\linewidth]{example-image-a}\\
\vspace{2pt}
\includegraphics[width=0.32\linewidth]{example-image-a}%
\hfill%
\includegraphics[width=0.32\linewidth]{example-image-a}%
\hfill%
\includegraphics[width=0.32\linewidth]{example-image-a}
\caption{\textbf{Tasks} \textit{Top row:} Simulation; \textit{Bottom row:} Real world. \textit{From left to right:} XX, YY and ZZ tasks; While similar enough to transfer prior knowledge between them, our simulation and real task versions present a considerable gap (Sec.~\ref{ss:s2rdiffs}) that we are able to bridge using language as regularization for the image representation}  
\label{fig:tasks}
\end{figure}

\subsection{Task Suite 1: Stack Object}
\label{sec:exp:stack}
In our first suite of tasks, the robot must move an object to a target. In the simulated domain $D^{(1)}$, the target is on top of a wooden coaster, and there are four objects, milk carton, soda can, bread, and cereal box, which correspond to the four tasks. Both the object and the coaster positions are randomized over the entire workspace. We collect and train on $400$ trajectories per task ($1600$ total) as our $D^{(1)}$ simulation data.
\begin{table*}[htbp]
  \centering
  \caption{Sim2Real}
  \begin{tabular}{cccccccccccccccc}
    \toprule
    Pretraining & \multicolumn{3}{c}{Action-labeled Data} &  \multicolumn{3}{c}{Move Carrot} & \multicolumn{6}{c}{Serve Carrot} & \multicolumn{3}{c}{Wrap Cord}\\
    \cmidrule(r{4pt}){2-4} \cmidrule(l){5-7} \cmidrule(l){8-13} \cmidrule(l){14-16}
    & & & & \multicolumn{3}{c}{success rate} & \multicolumn{3}{c}{success rate} & \multicolumn{3}{c}{subtasks completed} & \multicolumn{3}{c}{success rate} \\
    \cmidrule(l){5-7}\cmidrule(l){8-10}\cmidrule(l){11-13} \cmidrule(l){14-16}
    & Sim & Real $T^{(2)}$ & Real $T^{(2)}_{prior}$& 25 & 50 & 100 & 25 & 50 & 100 & 25 & 50 & 100 & 25 & 50 & 100 \\
    \midrule 
    
    None & -- & \ding{51} & \ding{51} & 45 & 30 & 65 & 40 & 20 & 30 & 1.15 & 0.9 & 1.15 &  25 & 45 & 35\\
    None & \ding{51} & \ding{51} & \ding{51} & 20 & 55 & 25 & 45 & 30 & 50 & 1.25 & 1.2 & 1.4 & 15 & 30 & 30 \\
    \midrule
    Lang Reg. (ours) & \ding{51} & \ding{51} & -- & 50 & 55 & \textbf{85} & 55 & \textbf{80} & \textbf{95} & 1.2 & \textbf{1.8} & \textbf{1.95} & 25 & \textbf{50} & 55\\
    Lang Dist. (ours) & \ding{51} & \ding{51} & -- & 30 & 65 & 70 & 25 & 50 & 65 & 0.95 & 1.4 & 1.5 & 15 & 25 & 60  \\
    Stage Classif. & \ding{51} & \ding{51} & -- & 70 & 60 & 70 & 20 & 60 & 85 & 0.9 & 1.5 & 1.8 & 15 & 20 & \textbf{70} \\
    CLIP (frozen) & \ding{51} & \ding{51} & \ding{51} & 30 & 25 & 35 & 25 & 45 & 35 & 0.55 & 0.95 & 0.95 & \textbf{35} & 40 & 45\\ 
    R3M (frozen) & \ding{51} & \ding{51} & \ding{51} & \textbf{80} & \textbf{70} & 80 & \textbf{75} & 75 & 85 & \textbf{1.6} & 1.55 & 1.75 & 30 & 25 & 20\\
    \bottomrule
  \end{tabular}
  \label{tab:real}
\end{table*}

\begin{table*}[htbp]
  \centering
  \setlength{\tabcolsep}{0.3em}
  \caption{Sim2Sim: Success Rate by task (\%) $\uparrow$}
  \begin{tabular}{ccccccccccccccc}
    \toprule
     
     Pretraining & \multicolumn{5}{c}{Stack Object} & \multicolumn{5}{c}{Multi-step Pick and Place} & Wrap Wire \\
    \cmidrule(l){2-6}
    \cmidrule(l){7-11}
    \cmidrule(l){12-12}
    & 1 & 2 & 3 & 4 & avg & 1 & 2 & 3 & 4 & avg & 1\\
    \midrule
    None ($\targetD$ data only) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    None ($\priorD + \targetD$ data)  & -- & -- & -- & -- & -- & $28.4 \pm 10.9$ & $31.3 \pm 10.7$ & $13.9 \pm 5.5$ & $27.8 \pm 10.2$ & -- & $82.1 \pm 6.8$  \\
    \midrule
    Lang Reg. (ours) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $90.7 \pm 5.4$   \\
    Lang Dist. (ours) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & --   \\
    Stage Classif. & -- & -- & -- & -- & -- & $63.1 \pm 9.9$ & -- & -- & -- & -- & $91.4 \pm 3.6$   \\
    CLIP (frozen) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & --  \\
    R3M (frozen) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    \bottomrule
  \end{tabular}
  \label{tab:sim}
\end{table*}
\subsubsection{\textbf{Sim2Sim}} For sim2sim experiments on this task suite, we define a new $D^{(2)}$ simulated environment with differences from $D^{(1)}$ as enumerated in Section~\ref{sec:exp:sim2simdiff}. In addition to the 1600 $D^{(1)}$ trajectories, we add 100 target task $(T^{(2)})$ trajectories in $D^{(2)}$. Note that $D^{(2)}$, like $D^{(1)}$, has the same four tasks that involve manipulating the four objects. We test transfer to each of these four tasks in $D^{(2)}$. Results are shown in the Stack Object section of Table~\ref{tab:sim}. Each column represents a different target task in $D^{(2)}$. [Analyze results]

\subsubsection{\textbf{Sim2real}} For sim2real, $D^{(1)}$ remains the same as sim2sim using 1600 trajectories between the four objects. $D^{(2)}$ is a real world environment in which the object is randomly placed on the left mat and the goal is to finish with the object on the right mat and the gripper open at the end of 20 timesteps. As a real world prior task $T^{(2)}_{prior}$, we collect 50 trajectories of moving a rectangular paper box from the left to the right mat. Our method pretrains on the images from these 50 prior task trajectories without any other $D^{(2)}$. Our results are shown in Table~\ref{tab:real}. R3M surpasses our method with lower amounts of target task data on this task, benefiting from a higher advantage to the additional action labeled prior task trajectories in the lowest data experiments. Additionally, we see that the V+L pretrained baselines, R3M and CLIP, plateau and do not reach as high of accuracy, and R3M doesn't perform as well on more complex tasks. classif, lang reg, and lang dist consistently outperforms the no pretraining baselines, showing it does help bridge the sim2real gap (Q1), but no clear effect of language over classification pretraining (Q3). The results indicate a benefit of language regression over language distance for this task (Q4).

% \begin{table}[htbp]
%   \centering
%   \caption{Real World: Move Carrot}
%   \begin{tabular}{ccccccc}
%     \toprule
%     Pretraining & \multicolumn{3}{c}{Action-labeled Data} &  \multicolumn{3}{c}{\shortstack{Success Rate \\ (\%) $\uparrow$}} \\
%     \cmidrule(r{4pt}){2-4} \cmidrule(l){5-7}
%     & & $T^{(2)}$ & $T^{(2)}_{prior}$ & \multicolumn{3}{c}{\# $T^{(2)}$ trajs.} \\
%     \cmidrule(l){5-7}
%     & Sim & Real & Real & 25 & 50 & 100 \\
%     \midrule
%     -- & -- & \ding{51} & \ding{51} & 45 & 30 & 65 \\
%     -- & \ding{51} & \ding{51} & \ding{51} & 20 & 55 & 25 \\
%     \midrule
%     Lang Reg. (ours) & \ding{51} & \ding{51} & -- & 50 & 55 & \textbf{85} \\
%     Lang Dist. (ours) & \ding{51} & \ding{51} & -- & 30 & 65 & 70 \\
%     Stage Classif. & \ding{51} & \ding{51} & -- & 70 & 60 & 70 \\
%     CLIP (frozen) & \ding{51} & \ding{51} & \ding{51} & 30 & 25 & 35 \\
%     R3M (frozen) & \ding{51} & \ding{51} & \ding{51} & \textbf{80} & \textbf{70} & 80 \\
%     \bottomrule
%   \end{tabular}
%   \label{tab:real-pp}
% \end{table}

%%%%%%%%%%%%%%
%%% TASK 2 %%%
%%%%%%%%%%%%%%

\subsection{Task Suite 2: Multi-step Pick and Place}
In our second suite of tasks, we test a longer-horizon manipulation task. In simulation, the robot must first put an object in the pot, then grasp the pot by its handle and move it onto the stove. We categorize this as a 2-step pick-and-place task since two pick-and-place operations must be executed successfully for overall task success. We use the same four object-task mappings from Section~\ref{sec:exp:stack}. The object, pot, and stove locations are all randomized within a quadrant of the workspace. Since this task is longer horizon, we train on more data---$1,400$ trajectories per task in $D^{(1)}$.
% so they are not initialized on top of each other

\subsubsection{\textbf{Sim2Sim}} Similar to the stacking task, in the sim2sim setting, we define a new $D^{(2)}$ environment with differences from $D^{(1)}$ enumerated in Section~\ref{sec:exp:sim2simdiff} and evaluate over the four tasks when given $100$ target-task $(T^{(2)})$ demonstrations in $D^{(2)}$. The baselines are also given $100$ prior task $T^{(2)}_{prior}$ action-labeled trajectories that our method does not have access to. Our results are shown in Table~\ref{tab:sim}. Across all four tasks, we see that our algorithm outperforms the non-pretrained baselines by $40\%$, nearly tripling the success rates. CLIP and R3M perform slightly better than the non-pretrained baselines but still achieve only half the success rate of our approach.

\subsubsection{\textbf{Sim2Real}} In the sim2real setup, we use the same $D^{(1)}$ data, while $D^{(2)}$ is the real environment. The target task $T^{(2)}$ is putting a carrot into a bowl, then putting the bowl onto a plate (see Figure~\ref{blah}). For real world prior task $T^{(2)}_{prior}$ data, we collect 50 trajectories of putting a wooden block into the bowl, and then stacking the bowl on the plate. Our real world results in Table~\ref{tab:real} show performance along two metrics. The first is success rate when trained on 25, 50, or 100 real world trajectories. A successful trajectory is one where the following three conditions are true after 50 timesteps: (1) the carrot is placed in the bowl, (2) the bowl is placed onto the plate, and (3) the gripper is opened. The second metric, number of subtasks completed, measures the average number of the two pick and place operations that the robot completed from the beginning---effectively a partial credit measure. For instance, if the robot only manages to finish the first subtask of putting the carrot in the bowl in the alloted number of time steps, that counts as 1 subtask completed. But if the robot completes the second subtask without completing the first subtask, that counts as 0 subtasks completed. Our methods outperform non-pretrained baselines by 10-45\% in success rate through all three amounts of target task trajectories (Q1). R3M performs best with the lowest data, with 75\% success compared to ours with 55\%, but ours increases to \%80 and \%95 on 50 and 100 trajectories respectively (Q2). In this task, language provides a substantial benefit of 10\%-35\% over classification across the experiments (Q3) and language regression consistently increases accuracy by 30\% compared to distance learning.

% \begin{table}[htbp]
%   \centering
%   \caption{Real World: Serve Carrot}
%   \begin{tabular}{ccccccccc}
%     \toprule
%     Pretraining & \multicolumn{2}{c}{Data} &  \multicolumn{6}{c}{Performance (by \# $T^{(2)}$ trajectories)} \\
%     \cmidrule(r{4pt}){2-3} \cmidrule(l){4-9}
%     &&& \multicolumn{3}{c}{\shortstack{Success Rate \\ (\%) $\uparrow$}} & \multicolumn{3}{c}{\shortstack{Subtasks Completed \\ (max 2) $\uparrow$}} \\
%     \cmidrule(l{4pt}r{4pt}){4-6} \cmidrule(l{4pt}){7-9}
%     & Sim & Real & 25 & 50 & 100 & 25 & 50 & 100 \\
%     \midrule
%     -- & -- & \ding{51} & 40 & 20 & 30 & 1.15 & 0.9 & 1.15 \\
%     -- & \ding{51} & \ding{51} & 45 & 30 & 50 & 1.25 & 1.2 & 1.4 \\
%     \midrule
%     Lang Reg. (ours) & \ding{51} & \ding{51} & 55 & \textbf{80} & \textbf{95} & 1.2 & \textbf{1.8} & \textbf{1.95} \\
%     Lang Dist. (ours) & \ding{51} & \ding{51} & 25 & 50 & 65 & 0.95 & 1.4 & 1.5 \\
%     Stage Classif. & \ding{51} & \ding{51} & 20 & 60 & 85 & 0.9 & 1.5 & 1.8 \\
%     CLIP (frozen) & \ding{51} & \ding{51} & 25 & 45 & 35 & 0.55 & 0.95 & 0.95 \\
%     R3M (frozen) & \ding{51} & \ding{51} & \textbf{75} & 75 & 85 & \textbf{1.6} & 1.55 & 1.75 \\
%     \bottomrule
%   \end{tabular}
%   \label{tab:real-obp}
% \end{table}


%%%%%%%%%%%%%%
%%% TASK 3 %%%
%%%%%%%%%%%%%%


\subsection{Task Suite 3: Wrap Wire around Appliance}
Our final suite of tasks involves wrapping a long deformable wire around a fixed object. In simulation $D^{(1)}$, we approximate a wire with a chain of spheres connected with free joints and use a cylinder in the middle of the table as the fixed object. The task is to wrap the chain around the cylinder. A trajectory is successful if the first link of the chain has traveled $\geq \frac{5\pi}{3}$ radians ($5/6$ths of a full revolution) around the cylinder. Our simulation data consists of two tasks: wrapping counterclockwise and clockwise. The initial position of the end of the chain is randomized over a region to the left of the cylinder, but the cylinder's position remains fixed between episodes. We collect 400 trajectories in each of the two tasks of $D^{(1)}$.

\subsubsection{\textbf{Sim2Sim}} For our $D^{(2)}$ sim environment, the two tasks are the same, but we again apply the changes specified in Section~\ref{sec:exp:sim2simdiff}. To widen the visual sim2sim gap, we make additional changes in $D^{(2)}$ by creating the chain out of capsules instead of spheres, and varying the color and texture of the cylinder, the robot, and the table. Our results are shown in Table~\ref{tab:sim}. [Analyze results.]

\subsubsection{\textbf{Sim2Real}} In our sim2real experiments, the target task $T^{(2)}$ in the real world domain $D^{(2)}$ is to first grasp the plug, then wrap the cord around the base of a blender in the middle of the workspace, and finally put the plug down. This is similar to what one might do before putting the appliance away in a cabinet. For real world prior task $T^{(2)}_{prior}$ data, we collect 50 trajectories of a similar wrapping task, except the plug, cord, and blender are replaced by a wooden block, ethernet cable, and spool, respectively.

We train on $D^{(1)}$ data and 25, 50, and 100 trajectories in the real world target task $T^{(2)}$ in $D^{(2)}$. Like the sim environment, we define success if the following two conditions are met: (1) the plug travels $\geq \frac{5 \pi }{3}$ radians around the blender, and (2) the object is placed and the gripper is open at the end of 50 timesteps. Results are shown in Table~\ref{tab:real-ww}. Note first that success rates on this task are lower across the board compared to previous tasks because the plug, as a small rigid object with a roughly 2cm $\times$ 5cm base, requires a higher degree of grasping precision than the larger soft carrot in the previous tasks.

While our method performs worse than CLIP and R3M in the low-data regime of 25 trajectories, it performs better than all pretrained and non-pretrained baselines [not counting stage classification] when trained on 50 or 100 target task trajectories. This demonstrates the effectiveness of \ouralgo{} in bridging the sim2real gap in tasks involving deformable object manipulation, which are hard to simulate with high fidelity. This answers our 3rd experimental question.

% \begin{table}[htbp]
%   \centering
%   \caption{Real World: Wrap Cord}
%   \begin{tabular}{cccccc}
%     \toprule
%     Pretraining & \multicolumn{2}{c}{Data} &  \multicolumn{3}{c}{\shortstack{Success Rate \\ (\%) $\uparrow$}} \\
%     \cmidrule(r{4pt}){2-3} \cmidrule(l){4-6}
%     & Sim & Real & 25 & 50 & 100 \\
%     \midrule
%     -- & -- & \ding{51} & 25 & 45 & 35 \\
%     -- & \ding{51} & \ding{51} & 15 & 30 & 30 \\
%     \midrule 
%     Lang Reg. (ours) & \ding{51} & \ding{51} & 25 & \textbf{50} & 55 \\
%     Lang Dist. (ours) & \ding{51} & \ding{51} & 15 & 25 & 60 \\
%     Stage Classif. & \ding{51} & \ding{51} & 15 & 20 & \textbf{70} \\
%     CLIP (frozen) & \ding{51} & \ding{51} & \textbf{35} & 40 & 45 \\
%     R3M (frozen) & \ding{51} & \ding{51} & 30 & 25 & 20 \\
%     \bottomrule
%   \end{tabular}
%   \label{tab:real-ww}
% \end{table}

\subsection{Summary and Overall Analysis}
Across the three task suites, we see that our method, which involves pretraining only on the images and language descriptions of a few hundred trajectories in sim and 50 trajectories in a prior task in the real domain, outperforms non-pretrained baselines in the few-shot sim2real setting in most of the data regimes tested. This demonstrates the robustness of our method in bridging wide sim2sim and sim2real gaps, answering our first experimental question. While CLIP is slightly better than R3M at wire wrapping and R3M outperforms CLIP on 2-step pick and place, our method achieves higher sim2real performance than the best of either pretrained baseline in both tasks, answering our second experimental question in the affirmative.


% \begin{table}[htbp]
%   \centering
%   \caption{Real World: Wrap Wire around Blender (with 2 sim tasks; ethernet cable bridge 3d printer spool in phase 1. p3 and p2+3 baselines already trained with action-labeled phase 1 data.}
%   \begin{tabular}{cccccc}
%     \toprule
%     Pretraining & \multicolumn{2}{c}{Data} &  \multicolumn{3}{c}{\shortstack{Success Rate \\ (\%) $\uparrow$}} \\
%     \cmidrule(r{4pt}){2-3} \cmidrule(l){4-6}
%     & Sim & Real & 25 & 50 & 100 \\
%     \midrule
%     -- & -- & \ding{51} & 20 & 25 & 35 \\
%     -- & \ding{51} & \ding{51} & 35 & 25 & 30 \\
%     \midrule
%     Lang Reg. (ours) & \ding{51} & \ding{51} & -- & -- & -- \\
%     Lang Dist. (ours) & \ding{51} & \ding{51} & -- & -- & -- \\
%     Stage Classif. & \ding{51} & \ding{51} & 35 & 25 & 50 \\
%     CLIP (frozen) & \ding{51} & \ding{51} & -- & -- & -- \\
%     R3M (frozen) & \ding{51} & \ding{51} & -- & -- & -- \\
%     \bottomrule
%   \end{tabular}
%   \label{tab:rwpp}
% \end{table}

% \subsection{Domains}
% \begin{itemize}
%     \item Sim2Real
%     \item (at the end) Sim2Sim
% \end{itemize}

% \subsection{Tasks}
% \begin{itemize}
%     \item Single-step
%     \item Multistep-step pick and place
%     \item Wire wrap
% \end{itemize}

% \subsection{Ablations}
% \begin{itemize}
%     \item Phase 2+3
%     \item Phase 3
%     \item Reduce number of stages in phase 1
%     \item Allow entire CNN to finetune in phase 2+3
% \end{itemize}

% \subsection{Our Method Phase 1 Comparisons}
% \begin{itemize}
%     \item Stage classification
%     \item Language Regression
%     \item BLEURT
% \end{itemize}

% \subsection{Baselines}
% \begin{itemize}
%     \item R3M Phase 2+3, 1 $\rightarrow$ 2+3
%     \item CLIP Phase 2+3, 1 $\rightarrow$ 2+3
%     \item MMD
% \end{itemize}

% \subsection{Metrics}
% \begin{itemize}
%     \item Success Rate by number of real world demos (25, 50, 100)
%     \item How many target-domain demos does it take for the baseline (Phase 2+3) to catch up to our method's performance?
% \end{itemize}


==> 06-experimental-results_0420.tex <==
Our results for \texttt{sim2sim} experiments are shown in Table~\ref{tab:sim}, and the results for \texttt{sim2real} are shown in Table~\ref{tab:real}. In both tables, the methods (rows) are grouped into non-pretrained baselines, our method variants and ablations, and pretrained SOTA baselines. In \texttt{sim2real}, we additionally include a group of three rows to show the performance of prior sim2real approaches.

\subsection{Experimental Questions and Analysis}
Across the three task suites in both \texttt{sim2real} and \texttt{sim2sim}, our method generally achieves the highest success rates.
% In particular, task suite 3 involves manipulating deformable objects, which is hard to simulate with high fidelity, widening the sim2real gap. We see lower success rates across the board but attribute this to small rigid plug (2cm $\times$ 5cm base) requiring a higher degree of grasping precision than the larger soft carrot in the previous tasks. Importantly, our method performs better than SOTA vision-language pretraining and non-pretrained baselines with wire wrap on 50 and 100 target task demonstrations on task suite 3, which demonstrates the effectiveness of \ouralgo{}.
% In general, we notice more pronounced differences between variants of our method and the  in sim2real, likely due to the larger domain gap.
% In sim2real, we evaluate on 3 levels of $\targetDtargetT$ data. In sim2sim we evaluate on 4 tasks for Task Suite 1 and 2. The predominant trends, however, do remain constant between sim2sim and sim2real.
To further analyze the effectiveness of our method, we pose and investigate the following four experimental questions.

\textit{\textbf{What is the impact of our pretraining approach?}}
Even without action-labeled $\targetDpriorT$ demonstrations that the baselines have access to, our method nearly doubles the success rate of both non-pretrained baselines in most task suites in \texttt{sim2real} and \texttt{sim2sim}. This indicates that \ouralgo{} can bridge a wide sim2real gap. One factor that may allow our method to perform well is that image observations with similar language descriptions may also have similar action labels. In the Appendix, we further investigate this hypothesis with an analysis of the action distributions between images, split by their language descriptions.

Between the non-pretrained baselines, training on $\priorD$ sim demonstrations in sim2real provides little benefit, decreasing performance by 10\% on stack object and wrap wire, but increasing by $\approx12\%$ on multi-step pick and place. However, in \texttt{sim2sim}, it provides a 10-15\% increase on most tasks. This suggests that the sim2sim gap is small enough to provide a benefit from using $\priorD$ even without pretraining, but that in \texttt{sim2real}, the gap is large enough that pretraining is required to leverage $\priorD$.
% The non-pretrained baseline using only $\targetD$ data $(\targetDpriorT \cup \targetDtargetT)$ and the second using $\targetD$ and $\priorD$ data, the $\priorD$ trajectories add little benefit without pretraining, given the large domain gap.

\textit{\rev{\textbf{How does our method compare to prior sim2real baselines?}}}
\rev{Our method outperforms all of the prior sim2real baselines (second row group in Table~\ref{tab:real}), which collectively do relatively poorly in most settings, highlighting the difficulty of the sim2real problem in our setup.}

\rev{MMD averages the best performance across the three sim2real baselines, and even achieves competitive performance on 2-step pick-and-place in the low-data regime. However, its performance does not scale well with more trajectories, which we suspect arises from stability issues in trying to push together the mean of all sim and real image embeddings in each batch. Domain randomization only exacerbates the sim2real gap as the implemented randomizations do not move the distribution of simulation trajectories closer to the real world trajectories due to the large visual dissimilarity between our simulation and real environments. ADR+RNA, which only randomizes the environment as much as possible without severely hurting the scripted policy performance, performs better on average than domain randomization, perhaps because the data is less diverse and easier to fit a policy to than the data from full-scale domain randomization.}

\textit{{\textbf{How does our method compare to prior vision-language pretrained representations?}}}
In \texttt{sim2real}, on the simpler pick-and-place tasks, R3M surpasses our method with 25 target task demonstrations, perhaps because of the additional 50 $\targetDpriorT$ demonstrations that our method does not train on. However, on 50 and 100 trajectories for the longer-horizon multi-step pick and place task, our method achieves higher sim2real performance than the best of either pretrained baseline. Additionally, we see that R3M and CLIP plateau and do not reach as high an accuracy as ours with more data, and R3M doesn't perform as well on more complex tasks like real-world wire wrap.
CLIP fairly consistently achieves 25-45\% accuracy across all real-world tasks, even over different amounts of $\targetDtargetT$ data. 

In \texttt{sim2sim}, our method outperforms R3M and CLIP across the board. Averaging the performance on stack and multi-step pick and place, our method outperforms R3M by 15-30\% and CLIP by 25-40\%. On the wrap wire task, our method and R3M perform comparably, probably because the task is quite a bit easier for all methods in simulation.

\textit{\textbf{What is the effect of language in learning shared representations?}}
We ablate the effect of language on our pretraining as the ``stage classification'' row in Tables~\ref{tab:real} and~\ref{tab:sim}, as mentioned in Section~\ref{exp-results:method-ablation}. In \texttt{sim2sim}, we see similar performance in language regression pretraining and classification pretraining. However, in \texttt{sim2real}, where the domain gap is larger, we see language providing a real benefit in multi-step pick and place, perhaps because the pretraining method leverages similarities in language descriptions between the first and second steps of the pick and place task.
 % , while also differentiating the objects in each subtask.
% Conversely, the classification baseline does not benefit as much and performs worse on task 2, showing the advantage of language.

\textit{\textbf{How do our two pretraining variants involving language compare?}}
We compare the two language pretraining methods introduced in Sections~\ref{sec:method:lang-reg} and~\ref{sec:method:lang-dist}, where language regression directly predicts language embeddings while language distance is encouraged to maintain pairwise distances based on BLEURT similarity scores. Again in \texttt{sim2sim}, there is no clear winner between the two, but in \texttt{sim2real}, we observe that language regression performs better on all three real task suites. This suggests that when performing language pretraining for visual representations, the more constraining regression loss outperforms the less constraining distance-matching loss on \texttt{sim2real} performance.

\textit{\textbf{\rev{What is the effect of pretraining on image-language pairs where the language granularity is reduced?}}}
\rev{We evaluate the impact of reduced language granularity on \texttt{sim2real} performance. See Appendix\ref{appendix:lang-granularity-results} for results.}

% This demonstrates that directly predicting the language embeddings is more successful than distance learning. The higher amount of constraint on the learned representation, and the additional structure imposed by language embeddings is helps to preserve more information and \_\_\_. 

%should we have a section on sim2sim vs sim2real

%better explanation this is not clear
% via directly predicting language embeddings compare to distance learning, in which the CNN is encouraged to maintaining the BLEURT similarity between language and images?


==> experiments-2-2-2023.tex <==
To investigate the effectiveness of our method, we pose the following questions:
\begin{enumerate}[start=1,label={Q\arabic*:}]
    \item Can \ouralgo{} help bridge a wide sim2real gap involving large differences in visual appearance, scene objects, task goals, and robot control frequency?
    \item How does \ouralgo{} compare to prior vision-language pretrained representations that have demonstrated success in downstream robotics applications?
    \item What is the impact of language in learning shared representations as opposed to to similar non-language based domain-specific pretraining?
    \item How does pretraining via directly predicting language embeddings compare to distance learning, in which the CNN is encouraged to maintaining the BLEURT similarity between language and images?
    
\end{enumerate}

We evaluate these questions across three task suites: (1) stacking an object on another, (2) cooking/serving food (multi-step pick and place), and (3) wrapping a cord around an appliance. For each task suite, we evaluate in both the sim2sim and sim2real settings. 

\subsection{Sim2Sim Environment Differences}
\label{sec:exp:sim2simdiff}
In sim2sim, the two sim environments $\priorD$ and $\targetD$ have the following differences:
\begin{enumerate}
    \item \textbf{Camera point-of-view}: $\priorD$ image observations are third person (looking toward the robot), and $\targetD$ image observations are first person (looking outward from above the robot arm's shoulder).
    \item \textbf{Friction and Damping}: Joint friction and damping coefficients are $5 \times$ and $50\times$ higher in $\targetD$ than $\priorD$.
    \item \textbf{Visual appearance}: For task suite 3 wrap wire, attributes including object and cylinder shape/color as well as table and gripper texture/color differ. Task suite 1 and 2 do not have this additional difference.
\end{enumerate}

\subsection{Sim2Real Environment Differences}
\label{ss:s2rdiffs}
The sim and real environments share state and action space dimensionality to enable a single policy to fit to data from both domains, but compared to prior work that requires significant engineering to reduce differences between the sim $\priorD$ and real $\targetD$ environment, we employ a setup with a wide sim2real gap including the following factors:
\begin{enumerate}
    \item \textbf{Control frequency}: The simulated $\priorD$ policy runs at 50Hz while the real world $\targetD$ policy runs at 2Hz.
    \item \textbf{Objects}: The objects on the scene in each task differ between simulation and real data, except the robot itself.
    \item \textbf{Visual Observation}: Backgrounds and camera angles are markedly different between the two domains.
    \item \textbf{Initial positions}: The initial object and robot positions are different across sim and real.
    \item \textbf{Action magnitude}: Real robot x, y, and z action are restricted so each are $\le 1$, and higher values are scaled before being executed. 
\end{enumerate}

\subsection{Baselines}
To evaluate the effectiveness of \ouralgo{}, we consider two sets of baselines: non-pretrained baselines where the CNN is initialized from scratch, and pre-trained baselines where the CNN is taken from recent vision+language works.
For the non-pretrained baselines, we examine training with only $\targetD$ data, and training with both $\priorD$ and $\targetD$ data.
For the pretrained baselines, we compare with using frozen CLIP~\cite{radford2021learning} and R3M~\cite{nair2022r3m} as the visual backbone, as both are commonly used visual representations for robotics and were shaped by language descriptions of images/videos.

In all our experiments, all baselines (non-pretrained and pretrained) are given access to $\targetD$ action-labeled data from two tasks: the target task $\targetDtargetT$ and prior task $\targetDpriorT$. Crucially, our method, on the other hand, is only given action-labeled data for $\targetDtargetT$. \textit{Our method is not given $\targetDpriorT$ action-labeled data} because it was trained on $\targetDpriorT$ images (with language labels) during image-language pretraining.(Section~\ref{sec:method:imglangpt}). Therefore, the baselines in a sense serve as upper-bounds because they are given 50 additional trajectories of action-labels in $\targetDpriorT$.

For each task, our experimental tables show results split by number of $\targetDtargetT$ trajectories, 25, 50, 100, which are shown as columns under each performance metric. This means that in terms of $\targetD$ action-labeled data, all baselines are trained on 75, 100, and 150 total trajectories, given the 50 additional $\targetDpriorT$ trajectories. Our method is only trained on the 25, 50, and 100 action-labeled trajectories from $\targetDtargetT$.

\subsection{Data}
Environments: For each of our tasks, we design simulation environments on top of robosuite~\citep{zhu2020robosuite} in mujoco~\citep{todorov2012mujoco}. For the real environment, we use Operational Space Control from deoxys. In both simulation and real, we work with a 7DOF Franka Emika Panda arm.

Both the sim and real environments have continuous xyz delta action space, and the gripper dimension is also continuous, ranging from $[-1, 0]$ to control the amount the gripper should be closed. The image observation space is $128 \times 128$ RGB images, and the state space is 22-dimensional, consisting of the robot's xyz end-effector position, gripper state, and sine and cosine transformations of the 7 joint angles.

For each task suite, we collect data from two domains: simulated domain $\priorD$ and target domain $\targetD$ (which is either another simulated domain or the real domain depending on whether we are doing sim2sim or sim2real transfer). All of our demonstrations in sim and real are collected with a scripted policy. Sim trajectories range from 200-320 timesteps long, as they operate at 50Hz, while real trajectories run at 2Hz and range from 18-45 timesteps in horizon length.


\begin{figure}[t!]
\centering
\includegraphics[width=0.32\linewidth]{simppm2.png}%
\hfill%
\includegraphics[width=0.32\linewidth]{simppx212.png}%
\hfill%
\includegraphics[width=0.32\linewidth]{simww12.png}\\
\vspace{2pt}
\includegraphics[width=0.32\linewidth]{realpp.png}%
\hfill%
\includegraphics[width=0.32\linewidth]{realppx2.png}%
\hfill%
\includegraphics[width=0.32\linewidth]{realw.png}\\
\vspace{2pt}
\includegraphics[width=0.32\linewidth]{simppt2.png}%
\hfill%
\includegraphics[width=0.32\linewidth]{simppx2t2.png}%
\hfill%
\includegraphics[width=0.32\linewidth]{simwwt2.png}

\caption{\textbf{Tasks} \textit{Top row:} Simulation $\priorD$; \textit{Middle row:} sim2real $\targetDtargetT$ \textit{Bottom row:} sim2sim $\targetDtargetT$ \textit{From left to right:} Stack Object, Multi-step Pick and Place, and Wrap Wire tasks; While similar enough to transfer prior knowledge between them, our simulation and real task versions present a considerable gap (Sec.~\ref{ss:s2rdiffs}) that we are able to bridge using language as regularization for the image representation}  
\label{fig:tasks}
\end{figure}

%%%%%%%%%%%%%%
%%% TASK 1 %%%
%%%%%%%%%%%%%%
\subsection{Task Suite 1: Stack Object}
\label{sec:exp:stack}
In our first suite of tasks, the robot must move an object to a target. In the simulated domain $\priorD$, the target is on top of a wooden coaster, and there are four objects, milk carton, soda can, bread, and cereal box, which correspond to the four tasks. Both the object and the coaster positions are randomized over the entire workspace. We collect and train on $400$ trajectories per task ($1600$ total) as our $\priorD$ simulation data.
\begin{table*}[htbp]
  \centering
  \caption{Sim2Real}
  \begin{tabular}{cccccccccccccccc}
    \toprule
    Pretraining & \multicolumn{3}{c}{Action-labeled Data} &  \multicolumn{3}{c}{Move Carrot} & \multicolumn{6}{c}{Serve Carrot} & \multicolumn{3}{c}{Wrap Cord}\\
    \cmidrule(r{4pt}){2-4} \cmidrule(l){5-7} \cmidrule(l){8-13} \cmidrule(l){14-16}
    & Sim & \multicolumn{2}{c}{Real} & \multicolumn{3}{c}{success rate} & \multicolumn{3}{c}{success rate} & \multicolumn{3}{c}{subtasks completed} & \multicolumn{3}{c}{success rate} \\
    \cmidrule(l){5-7}\cmidrule(l){8-10}\cmidrule(l){11-13} \cmidrule(l){14-16}
    &  ($\priorD$) &  $\targetDtargetT$ &  $\targetDpriorT$& 25 & 50 & 100 & 25 & 50 & 100 & 25 & 50 & 100 & 25 & 50 & 100 \\
    \midrule 
    
    None ($\targetD$ data only) & -- & \ding{51} & \ding{51} & 45 & 30 & 65 & 40 & 20 & 30 & 1.15 & 0.9 & 1.15 &  25 & 45 & 35\\
     None ($\priorD + \targetD$ data) & \ding{51} & \ding{51} & \ding{51} & 20 & 55 & 25 & 45 & 30 & 50 & 1.25 & 1.2 & 1.4 & 15 & 30 & 30 \\
    \midrule
    Lang Reg. (ours) & \ding{51} & \ding{51} & -- & 50 & 55 & \textbf{85} & 55 & \textbf{80} & \textbf{95} & 1.2 & \textbf{1.8} & \textbf{1.95} & 25 & \textbf{50} & 55\\
    Lang Dist. (ours) & \ding{51} & \ding{51} & -- & 30 & 65 & 70 & 25 & 50 & 65 & 0.95 & 1.4 & 1.5 & 15 & 25 & 60  \\
    Stage Classif. & \ding{51} & \ding{51} & -- & 70 & 60 & 70 & 20 & 60 & 85 & 0.9 & 1.5 & 1.8 & 15 & 20 & \textbf{70} \\
    CLIP (frozen) & \ding{51} & \ding{51} & \ding{51} & 30 & 25 & 35 & 25 & 45 & 35 & 0.55 & 0.95 & 0.95 & \textbf{35} & 40 & 45\\ 
    R3M (frozen) & \ding{51} & \ding{51} & \ding{51} & \textbf{80} & \textbf{70} & 80 & \textbf{75} & 75 & 85 & \textbf{1.6} & 1.55 & 1.75 & 30 & 25 & 20\\
    \bottomrule
  \end{tabular}
  \label{tab:real}
\end{table*}

\begin{table*}[htbp]
  \centering
  \setlength{\tabcolsep}{0.3em}
  \caption{Sim2Sim: Success Rate by Task (\%) $\uparrow$}
  \begin{tabular}{ccccccccccccccc}
    \toprule
     
     Pretraining & \multicolumn{5}{c}{Stack Object} & \multicolumn{5}{c}{Multi-step Pick and Place} & Wrap Wire \\
    \cmidrule(l){2-6}
    \cmidrule(l){7-11}
    \cmidrule(l){12-12}
    & 1 & 2 & 3 & 4 & avg & 1 & 2 & 3 & 4 & avg & 1\\
    \midrule
    None ($\targetD$ data only) & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    None ($\priorD + \targetD$ data)  & -- & -- & -- & -- & -- & $28.4 \pm 10.9$ & $31.3 \pm 10.7$ & $13.9 \pm 5.5$ & $27.8 \pm 10.2$ & -- & $82.1 \pm 6.8$  \\
    \midrule
    Lang Reg. (ours) & $20.6 \pm 8.1$ & $57.3 \pm 8.1$ & $63.1 \pm 7.7$ & -- & -- & $54.0 \pm 7.2$ & \boldmath{$62.5 \pm 12.1$} & $76.0 \pm 8.7$ & -- & -- & $90.7 \pm 5.4$   \\
    Lang Dist. (ours) & -- & -- & -- & -- & -- & \boldmath{$65.5 \pm 13.1$} & $56.7 \pm 9.9$ & -- & $54.4 \pm 11.5$ & -- & --   \\
    Stage Classif. & -- & -- & -- & -- & -- & $63.1 \pm 9.9$ & $62.1 \pm 9.3$ & $55.4 \pm 8.5$ & $67.7 \pm 9.7$ & -- & $91.4 \pm 3.6$   \\
    CLIP (frozen) & -- & -- & -- & -- & -- & $36.1 \pm 14.3$ & $39.9 \pm 8.9$ & -- & -- & -- & $75.6 \pm 7.7$  \\
    R3M (frozen) & -- & -- & -- & -- & -- & $49.4 \pm 11.6$ & $36.5 \pm 11.9$ & $47.0 \pm 14.1$ & $56.0 \pm 10.0$ & -- & $90.2 \pm 4.4$ \\
    \bottomrule
  \end{tabular}
  \label{tab:sim}
\end{table*}
\subsubsection{\textbf{Sim2Sim}} For sim2sim experiments on this task suite, we define a new $\targetD$ simulated environment with differences from $\priorD$ as enumerated in Section~\ref{sec:exp:sim2simdiff}. In addition to the 1600 $\priorD$ trajectories, we add 100 target task $\targetDtargetT$. Note that $\targetD$, like $\priorD$, has the same four tasks that involve manipulating the four objects. We test transfer to each of these four tasks in $\targetD$. 

\subsubsection{\textbf{Sim2real}} For sim2real, $\priorD$ remains the same as sim2sim using 1600 trajectories between the four objects. $\targetD$ is a real world environment in which the object is randomly placed on the left mat and the goal is to finish with the object on the right mat and the gripper open at the end of 20 timesteps. As a real world prior task $\targetDpriorT$, we collect 50 trajectories of moving a rectangular paper box from the left to the right mat. Our method pretrains on the images from these 50 prior task trajectories without any other $\targetD$.

%%%%%%%%%%%%%%
%%% TASK 2 %%%
%%%%%%%%%%%%%%

\subsection{Task Suite 2: Multi-step Pick and Place}
In our second suite of tasks, we test a longer-horizon manipulation task. In simulation, the robot must first put an object in the pot, then grasp the pot by its handle and move it onto the stove. We categorize this as a 2-step pick-and-place task. We use the same four object-task mappings from Section~\ref{sec:exp:stack}. The object, pot, and stove locations are all randomized within a quadrant of the workspace. Since this task is longer horizon, we train on more data---$1,400$ trajectories per task in $\priorD$.

\subsubsection{\textbf{Sim2Sim}} Similar to the stacking task, in the sim2sim setting, we define a new $\targetD$ environment with differences from $\priorD$ enumerated in Section~\ref{sec:exp:sim2simdiff} and evaluate over the four tasks when given $100$ target-task $\targetDtargetT$ demonstrations. The baselines are also given $100$ prior task $\targetDpriorT$ action-labeled trajectories which our method does not have access to.


\subsubsection{\textbf{Sim2Real}} In the sim2real setup, we use the same $D^{(1)}$ data, while $D^{(2)}$ is the real environment. The target task $T^{(2)}$ is putting a carrot into a bowl, then putting the bowl onto a plate (see Figure~\ref{blah}). For real world prior task $T^{(2)}_{prior}$ data, we collect 50 trajectories of putting a wooden block into the bowl, and then stacking the bowl on the plate. Our real world results in Table~\ref{tab:real} show performance along two metrics. The first is success rate, defined by the the following three conditions being true after 50 timesteps: (1) the carrot is placed in the bowl, (2) the bowl is placed onto the plate, and (3) the gripper is opened. The second metric, number of subtasks completed, measures the average number of the two pick and place operations that the robot completed from the beginning---effectively a partial credit measure. If the robot completes the full task, it completes two subtasks, but if it only finishes the first subtask of putting the carrot in the bowl, it receives credit for 1 subtask. Completing the second without completing the first and completing neither both count as 0 complete subtasks. 


\subsection{Task Suite 3: Wrap Wire around Appliance}
Our final suite of tasks involves wrapping a long deformable wire around a fixed object. In simulation $D^{(1)}$, we approximate a wire with a chain of spheres connected with free joints and use a cylinder in the middle of the table as the fixed object. The task is to wrap the chain around the cylinder. A trajectory is successful if the first link of the chain has traveled $\geq \frac{5\pi}{3}$ radians ($5/6$ths of a full revolution) around the cylinder. Our simulation data consists of two tasks: wrapping counterclockwise and clockwise. The initial position of the end of the chain is randomized over a region to the left of the cylinder, but the cylinder's position remains fixed between episodes. We collect 400 trajectories of each of the two tasks in $D^{(1)}$. 

\subsubsection{\textbf{Sim2Sim}} For our $D^{(2)}$ sim environment, the two tasks are the same, but we again apply the changes specified in Section~\ref{sec:exp:sim2simdiff}, including the additional visual changes in $D^{(2)}$. This task involves a wider sim2sim gap, given additional visual changes and dynamics changes from the alternate shapes.

\subsubsection{\textbf{Sim2Real}} In our sim2real experiments, the target task $T^{(2)}$ in the real world domain $D^{(2)}$ is to first grasp the plug, then wrap the cord around the base of a blender in the middle of the workspace, and finally put the plug down, similar to what one might do before putting the appliance away. For real world prior task $T^{(2)}_{prior}$ data, we collect 50 trajectories of a similar wrapping task, except the plug, cord, and blender are replaced by a wooden block, ethernet cable, and spool, respectively.

We train on $D^{(1)}$ data and 25, 50, and 100 trajectories in the real world target task $T^{(2)}$ in $D^{(2)}$, and as with previous tasks, the baselines receive action-labeled $T^{(2)}_{prior}$ data. Like the sim environment, we define success if the following two conditions are met: (1) the plug travels $\geq \frac{5 \pi }{3}$ radians around the blender, and (2) the object is placed and the gripper is open at the end of 50 timesteps. 

\subsection{Summary and Overall Analysis}
Our results for sim2sim experiments are shown in Table~\ref{tab:sim} and the results for sim2real are shown in Table~\ref{tab:real}.
Across the three task suites, we see that our method, which involves pretraining only on the images and language descriptions of a few hundred trajectories in sim and 50 trajectories in a prior task in the real domain, outperforms non-pretrained baselines in the few-shot sim2real setting in most of the data regimes tested. This demonstrates the robustness of our method in bridging wide sim2sim and sim2real gaps (Q1).

\subsection{Task Differences}
While most of the trends we see between tasks are consistent, there are a few notable differences due to the nature of the tasks. First, for task suite 3, wire wrap, success rates are lower across the board because the plug is small (2cm $\times$ 5cm base) and rigid requires a higher degree of grasping precision than the larger soft carrot in the previous tasks. Additionally, our method performs better than SOTA vision-language pretraining and non-pretrained baselines with wire wrap on 50 and 100 target task trajectories on task suite 3, which demonstrates the effectiveness of \ouralgo{} in bridging the sim2real gap in tasks involving deformable object manipulation, which are hard to simulate with high fidelity.

\subsection{No Pretraining}
Our method performs at least well as both no pretraining baselines on every experiment, exceeding them on most, demonstrating that \ouralgo{} can bridge a wide sim2real gap (Q1). Additionally, between the two no pretraining baselines, the first using $T^{(2)}$ and $T^{(2)}_{prior}$ data and the second using $T^{(2)}$, $T^{(2)}_{prior}$, and $D^{(1)}$ data, the $D^{(1)}$ trajectories add little benefit without pretraining, given the large domain gap. 

\subsection{Vision-Language Pretrained Baselines}
R3M surpasses our method with low amounts of target task data, benefiting from a higher advantage to the additional action labeled prior task trajectories in the lowest data experiments. However, this effect is most pronounced for the simplest tasks and with 50 and 100 trajectories, our method achieves higher sim2real performance than the best of either pretrained baseline (Q2). Additionally, we see that R3M and CLIP plateau and do not reach as high of accuracy, and R3M doesn't perform as well on more complex tasks. 
CLIP performs fairly relatively consistently across all tasks, despite their differing nature and differing amounts of $D^{(2)}$ data, achieving 25-45\% accuracy.

\subsection{Task-specific pretraining}
We have three task-specific pretraining objectives: language regression, language distance, and stage classification. These three achieve the highest success with 50 and 100 trajectories, and perform better than all other baselines for these, and better than the non-pretraining baselines with 25 trajectories. More specifically, on task suite 1, move carrot, language regression performs best with 85\% on 100 trajectories, while stage classification does better than language regression on 25 and 50 trajectories for this task. Again on task 2, language regression achieves the highest success, aside from R3M on 25 trajectories. On task 3, language regression is most successful at 50\% with 50 trajectories and stage classification at 70\% on 100 trajectories. 

Between language regression and distance learning, lang reg performs better on all three tasks. This demonstrates that directly predicting the language embeddings is more successful than distance learning (Q4).

Comparing language regression and classification, we see similar performance on task suite 1 and higher performace from language regression on task suite 3. Language regression performs much better on the serve carrot task, than the simpler move carrot task, going from 25-55\% on 25 trajectories and 85-95\% with 100. It's able to effectively use the similarities between the first and second pick and place task, while also differentiating the objects in each subtask. Despite the fact that task 2 is harder than task 1, these features of language allows the language regression pretraining to benefit from the data in both pick and place subtasks and achieve higher success on task 2 than task 1. Conversely, the classification baseline does not benefit as much and performs worse on task 2, showing the advantage of language (Q3).
\\
